Robust Network Topology Inference and Processing of Graph Signals

The abundance of large and heterogeneous systems is rendering contemporary data more pervasive, intricate, and with a non-regular structure. With classical techniques facing troubles to deal with the irregular (non-Euclidean) domain where the signals are defined, a popular approach at the heart of graph signal processing (GSP) is to: (i) represent the underlying support via a graph and (ii) exploit the topology of this graph to process the signals at hand. In addition to the irregular structure of the signals, another critical limitation is that the observed data is prone to the presence of perturbations, which, in the context of GSP, may affect not only the observed signals but also the topology of the supporting graph. Ignoring the presence of perturbations, along with the couplings between the errors in the signal and the errors in their support, can drastically hinder estimation performance. While many GSP works have looked at the presence of perturbations in the signals, much fewer have looked at the presence of perturbations in the graph, and almost none at their joint effect. While this is not surprising (GSP is a relatively new field), we expect this to change in the upcoming years. Motivated by the previous discussion, the goal of this thesis is to advance toward a robust GSP paradigm where the algorithms are carefully designed to incorporate the influence of perturbations in the graph signals, the graph support, and both. To do so, we consider different types of perturbations, evaluate their disruptive impact on fundamental GSP tasks, and design robust algorithms to address them.

==> org_inicial.tex <==
% \section*{Posibles contenidos}
% Temas que pueden entrar como procesamiento robusto:
% \begin{itemize}
%     \item Ruido en la señal. Papers de denoising: \textbf{1J (submitted), 1C}.
%     \item Observaciones incompletas. Papers de topology inference with hidden: \textbf{1J (segundo autor), 2C + 1 in progress}.
%     \item Errores en la topología observada. Papers robust filter ID: \textbf{1C, 1J (in progress).}, paper sobre robust GNN \textbf{1C}.
% \end{itemize}

% Temas que podríamos relacionar pero son más tangenciales:
% \begin{itemize}
%     \item Muestreo: difícil de encajar pero \textbf{único journal aceptado}. Tal vez al hablar de "ruido en las señales"? Plantear como no observar todos los instantes.
    
%     \item Paper de motifs: una forma de hacer más robusta la inferencia de topología es con mejores priors. Por ahora solo con observaciones en todo el grafo, dejar como futuros trabajos observaciones con hidden.
    
%     \item Encoder/Decoder NNs: podríamos introducirlo como muestra de que la arquitectura decoder no es útil exclusivamente en el entorno de denoising (poco importante).
% \end{itemize}

% Imperfecciones pueden estar en forma de ruido o de información que falta. Esto puede ser en el shift o en las señales.

% La introducción debería ser amplia. Presentar varios problemas, introducir robustez en ellos.

% Al final de cada capítulo pensar como generalziarlo a otros setups?? (worth it?)

% \clearpage

\chapter*{Structure and highlights}

\section*{Acknowledgments / Agradecimientos}
Include funding here? Language?

\section*{Resumen}
El resumen debe presentarse encuadernado con la tesis doctoral.
4 páginas en la tesis de Miguel Ángel.
\begin{itemize}
    \item Antecedentes
    \item Objetivos
    \item Metodología
    \item Resultados
    \item Conclusiones
\end{itemize}


\section*{Abstract}
Should this be like the abstract from a paper but longer?
More details in the introduction and clearly emphasize objectives and contributions.

\section{Introduction}
Brief description of this chapter.

\begin{enumerate}
    % En las intros de las secciones puede ser bueno recordar los papers relacionados 
    \item Objectives. Our general goal is to approach fundamental problems from the GSP framework from a robust perspective. We want to deal with the different types of perturbations, always from a ``robust GSP'' perspective.
    \begin{itemize}
        \item When the signals are perturbed: propose non-linear denoising alternatives (vs classical method) to perform graph signal denoising when we face noise. (1 JCR, 1 Conf about denoising)
        \begin{itemize}
            \item Highlight the non-linear architecture is also useful for processing signals defined on different domains (graphs). [A subsection with the conferences may be to much but at least I would add a few paragraphs]. (If considered, 2 Conf of graph In/Out)
        \end{itemize}
        
        \item When the signal is perturbed because of the missing observations we need to reconstructed: introduce the sampling/reconstruction paper. (1 JCR about Sampling)
        
        \item When we have hidden nodes: learn the topology of the observed subgraph while taking into account the presence of hidden nodes. (1 JCR, 3 Conf) [Hablar si incluir el JCR, a lo mejor perjudica a Andrei]
        \begin{itemize}
            \item Talk about using better priors. Prior work in the Motif learning paper, idea to extend it to hidden nodes. Maybe not a subsection but a few paragraphs? (1 JCR) (Contribuciones adicionales?)
        \end{itemize}
        
        \item Approach classical GSP tasks while taking into consideration the perturbations in the observed topology. We focus on graph filter identification (1 JCR, 1 Conf about RFI).
    \end{itemize}
    Tal vez pensar algunos objetivos más genéricos / transversales -> otra "categoría". Especificar que estos son los objetivos más espécificos.
    
    \item Summary of contributions: enumerate the contributions and relate them with the different topics (objectives).

    \item Outline of the Thesis: brief description of the topic and structure of each chapter. Cortito.

\end{enumerate}


\section{Fundamentals of GSP}
Something like a compilation of Section~II in most of the papers involved.
\begin{itemize}
    \item Describe graph and graph signals
    \item Describe GSOs
    \item Main tools from GSP used in our papers: filters, frequency representation, stationarity, smoothness
\end{itemize}


\section{Perturbations in the signals}
Si no lo hago en la intro, motivar aquí el uso de arquitectura lineal y hablar de modelos clásicos. 
Lo mismo con el de sampling. Muchos esquemas de interpolación tnato lineales como no-lineales. Cosas del cap. anterior podrían extenderse aquí (underparametrized decoder).
Insistir ámbito muy trabajado, nuestra contribición es esta.
\begin{itemize}
    \item Short intro
    \item Imperfections as noise: Deep decoder
    \begin{itemize}
        \item \blue{Comment the Enc/Dec papers as other applications of the architecture? Maybe an approach robust to ``different domains''?} 
    \end{itemize}
    \item Imperfections as missing information: Sampling
    \item Generalizations to other setups: other inverse problems, sampling with uncertainty in the topology?
\end{itemize}


\section{Perturbations in the observed variables}
\begin{itemize}
    \item Short intro
    \item Main work: journal about hidden variables
    \item Extension to joint approaches
    \item Generalizations to other setups: topology inference driven by motif similarity (kind of a ``robust prior'' in the sense that allows comparing graphs of different sizes?) Maybe left Joint GMRF conference for this?
\end{itemize}

%Include paper of topology inference driven by motif similarity (kind of a ``robust prior'' in the sense that allows comparing graphs of different sizes?)

\section{Perturbations in the observed topology}
\begin{itemize}
    \item Short intro
    \item Main work: journal robust graph filter identification
    \item Application to non-linear problems: robust graph filters for GNN
    \item Generalizations to other setups: consider perturbations in the topology to other GSP problems (blind deconvolution? Sampling?)
\end{itemize}


\section{Conclusiones y Lineas futuras}
Resumen con insight adicional (no repetitivas)



